Reasoning with belief functions over Belnap--Dunn logic

We design an expansion of Belnap--Dunn logic with belief and plausibility functions that allow non-trivial reasoning with inconsistent and incomplete probabilistic information. We also formalise reasoning with non-standard probabilities and belief functions in two ways. First, using a calculus of linear inequalities, akin to the one presented in~\cite{FaginHalpernMegiddo1990}. Second, as a two-layered modal logic wherein reasoning with evidence (the outer layer) utilises paraconsistent expansions of \L{}ukasiewicz logic. The second approach is inspired by~\cite{BaldiCintulaNoguera2020}. We prove completeness for both kinds of calculi and show their equivalence by establishing faithful translations in both directions.

==> macros.tex <==
\newcommand{\redbf}[1]{\textcolor{red}{\textbf{#1}}}
\newcommand{\red}[1]{\textcolor{red}{{#1}}}
\newcommand{\bluebf}[1]{\textcolor{blue}{\textbf{#1}}}
\newcommand{\blue}[1]{\textcolor{blue}{{#1}}}
\usepackage{tikz}
\newcommand{\pl}{\mathtt{pl}}
\newcommand{\poss}{\mathtt{poss}}
\newcommand{\Pl}{\mathsf{Pl}}
\newcommand{\Prop}{\mathtt{Prop}}
\newcommand{\Sf}{\mathtt{Sf}}
\newcommand{\LIT}{\mathsf{Lit}}
\newcommand{\Prob}{\mathsf{Pr}}
\newcommand{\Bell}{\mathsf{Bel}}
\newcommand{\Plaus}{\mathsf{Pl}}
\newcommand{\bel}{\mathtt{bel}}
\newcommand{\Bel}{\mathtt{Bel}}
\newcommand{\belmod}{\mathsf{B}}
\newcommand{\mainL}{{\cal{L}}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\BD}{\mathsf{BD}}
\newcommand{\ETL}{\mathsf{ETL}}
\newcommand{\N}{\mathsf{N}}
\newcommand{\DS}{\mathsf{DS}}
\newcommand{\LBD}{\mathscr{L}_\mathsf{BD}}
\newcommand{\LTBD}{\mathcal{L}_\mathsf{BD}}
\newcommand{\Langluk}{\mathscr{L}_{\Luk^2}}
\newcommand{\Langluka}{\mathscr{L}_{\Luk}}
\newcommand{\LanglukN}{\mathscr{L}_{\N\Luk}}
\newcommand{\LatBD}{\mathcal{L}_\BD}
\newcommand{\LbBD}{\LBD^*}
\newcommand{\pr}{\mathtt{p}}
\newcommand{\mass}{\mathtt{m}}
\newcommand{\mf}{\mathtt{m}_f}
\newcommand{\mftb}{(\mf)_{\bot}^{\top}}
\newcommand{\f}{\varphi}
\newcommand{\p}{\psi}
\newcommand{\fDNF}{\mathsf{fDNF}}
\newcommand{\iDNF}{\mathsf{iDNF}}
\newcommand{\DNF}{\mathsf{DNF}}
\newcommand{\CNF}{\mathsf{CNF}}
\newcommand{\NNF}{\mathsf{NNF}}
\newcommand{\Luk}{{\mathchoice{\mbox{\rm\L}}{\mbox{\rm\L}}{\mbox{\rm\scriptsize\L}}{\mbox{\rm\tiny\L}}}}
\newcommand{\weakrightarrow}{\rightarrowtriangle}
\newcommand{\LNelson}{\Luk^2_{(1,1)^\uparrow}(\rightarrowtriangle)}
\newcommand{\LNelsonDelta}{\Luk^2_{(1,1)^\uparrow}(\rightarrowtriangle,\triangle)}
\newcommand{\Lsquaretop}{\Luk^2_{(1,0)}(\rightarrow)}
\newcommand{\LsquaretopDelta}{\Luk^2_{(1,0)}(\rightarrow,\triangle)}
\newcommand{\triangletop}{{\triangle^{\top}}}
